Imagine This! Scripts to Compositions to Videos

Imagining a scene described in natural language with realistic layout and appearance of entities is the ultimate test of spatial, visual, and semantic world knowledge. Towards this goal, we present the Composition, Retrieval, and Fusion Network (CRAFT), a model capable of learning this knowledge from video-caption data and applying it while generating videos from novel captions. CRAFT explicitly predicts a temporal-layout of mentioned entities (characters and objects), retrieves spatio-temporal entity segments from a video database and fuses them to generate scene videos. Our contributions include sequential training of components of CRAFT while jointly modeling layout and appearances, and losses that encourage learning compositional representations for retrieval. We evaluate CRAFT on semantic fidelity to caption, composition consistency, and visual quality. CRAFT outperforms direct pixel generation approaches and generalizes well to unseen captions and to unseen video databases with no text annotations. We demonstrate CRAFT on FLINTSTONES, a new richly annotated video-caption dataset with over 25000 videos. For a glimpse of videos generated by CRAFT, see https://youtu.be/688Vv86n0z8.

==> sections/background_retriever.tex <==
\section{Background Retriever}
The background retrieval

==> sections/entity_retriever.tex <==
\section{Entity Retriever} 
The task of the entity retriever is to find an entity in the target database which matches the description \emph{and} is consistent with the video constructed so far -- the video with all previous entities retrieved and placed in the respective locations predicted by the layout network. We adopt an embedding based lookup approach for entity retrieval. The query and database embedding networks are learned using the query-target pairs $\left<(T^{[m]},e_i^{[m]},l_i^{[m]},V_{i-1}^{[m]}),(V^{[m]},l_i^{[m]},s_i^{[m]})\right>_{i,m}$ in the training data. We denote the networks embedding the query and targets as $Q$ and $R$ respectively. For clarity, we abbreviate $Q(T^{[m]},e_i^{[m]},l_i^{[m]},V_{i-1}^{[m]})$ as $q_i^{[m]}$ and $R(V^{[m]},l_i^{[m]},s_i^{[m]})$  as $r_i^{[m]}$. At each training iteration, we sample a mini-batch of $B$ pairs without replacement and compute embeddings $\{(q_{i_b}^{[m_b]},r_{i_b}^{[m_b]})\}_{b=1}^{B}$ where $q$ and $r$ are each sequence of $F$ embeddings corresponding to $F$ video frames. The model is trained using a triplet loss computed on \emph{all possible} triplets in the mini-batch. Let $\delta_b$ denote the set of all indices from $1$ to $B$ except $b$. The loss can then be defined as 
\begin{multline}
\mathcal{L}_{triplet} = \frac{1}{B\cdot(B-1)}\sum_{b=1}^{B}\sum_{b^-\in \delta_b} \left[ \max(0,\gamma + q_{i_b}^{[m_b]}\odot r_{i_{b^-}}^{[m_{b^-}]} - q_{i_b}^{[m_b]}\odot r_{i_{b}}^{[m_{b}]}) \; + \right. \\
\left. \max(0,\gamma + q_{i_{b^-}}^{[m_{b^-}]}\odot r_{i_b}^{[m_b]} - q_{i_b}^{[m_b]}\odot r_{i_{b}}^{[m_{b}]})
\right]
\end{multline}
where $q\odot r=\frac{1}{F}\sum_{f=1}^{F}q[f] \cdot r[f]$ is the average dot product between corresponding query and target frame embeddings. 

\subsection{Auxiliary Multi-label Classification Loss}
We found models trained using triplet loss alone suffered from poor generalization to unseen captions and database videos. To guide the learning to capture semantics, we added an auxiliary classification loss on top of the embeddings. The key idea is to enrich the semantics of the embedding vectors by predicting the noun, adjectives, and action words directly associated with the entity in the description. A vocabulary $\mathcal{W}$ is constructed of all nouns, adjectives and verbs appearing in the training data. Then for each sample in the mini-batch, an MLP is used as a multi-label  classifier to predict associated words from the query and target embeddings. Let $P_{aux}(w|v)$ denote the probability of word $w$ given an embedding vector $v$. If $\mathcal{W}_i$ is the set of words associated with entity $E_i$, then the auxiliary loss is defined by
\begin{multline}
\mathcal{L}_{aux} = \sum_{b=1}^{B}
\left[
\sum_{w\in \mathcal{W}_{i_b}} -\;\log(P_{aux}(w|q_{i_{b}}^{[m_b]})) - \log(P_{aux}(w|r_{i_{b}}^{[m_b]})) \; + \right. \\
\left.
\sum_{w\in \mathcal{W}\setminus \mathcal{W}_{i_b}} -\;\log(P_{aux}(w|q_{i_{b}}^{[m_b]})) - \log(P_{aux}(w|r_{i_{b}}^{[m_b]}))
\right]
\end{multline}
Note that the same MLP is used to make predictions on both query and target embeddings.

\subsection{Entity Retriever Network Architecture}

\subsubsection{Query Embedding Network.} Similar to layout predictor's feature computation backbone, the query embedding network consist of a CNN to independently encode every frame of $V_{i-1}$ and an LSTM to encode $(T,e_i)$ which are concatenated together along with a 2-D coordinate grid to get per-frame feature maps. However, unlike layout predictor, query embedding network also needs to be conditioned on the position $l_i$ where entity $E_i$ is going to be inserted in $V_{i-1}$. To get location and scale specific query embeddings, we use a simplified RoIAlign (RoIPool with RoI quantization but with bilinear interpolation) mechanism to crop out the per-frame feature maps using the corresponding bounding box $l_i^f$ and scaling it to a $7\times7$ receptive field. The RoIAlign features are then averaged along the spatial dimensions to get the vector representations for each time step independently. An LSTM applied over the sequence of these embeddings is used to capture temporal context. The hidden output of the LSTM at each time step is normalized and used as the frame query embedding $q[f]$. 

\subsubsection{Target Embedding Network.} Since during inference, the target network needs to embed entities in the target database, which does not have text annotations, this network does not use $T$ as an input. Thus, the target embedding network is similar to the query network but without the LSTM to encode the text. We are also only interested in representing the pixels that belong to the entity being considered for retrieval. Hence the video is masked by the corresponding segmentation mask before feeding into the network. In our experiments we found that using 2-D coordinate features in both query and target networks made the network susceptible to ignoring all other features since it provides an easy signal for matching ground truth query-target pairs during training. This in turn leads to poor generalization. Thus, we remove the 2-D coordinate features from the target network.




==> sections/introduction_backup.tex <==
\input{figures/hero.tex}
\section{Introduction}


Consider the scene description: \emph{Fred is wearing a blue hat and talking to Wilma in the living room. Wilma then sits down on a couch}. Picturing the scene in our mind requires the knowledge of plausible locations, appearances, actions, and interactions of characters and objects being described as well as an ability to understand and translate the natural language description into a plausible visual instantiation. In this work, our goal is to jointly model the layout and appearance of entities in complex scenes from paired video-caption data and to apply this learned knowledge to generate plausible videos from novel text descriptions. To systematically make progress towards this goal we introduce the task of \taskfull\ and a richly annotated dataset, \dataset.

Modelling the layout and appearances of entities for descriptions like the one above poses several challenges: (a) \textbf{Entity Recall} - the video must contain the relevant characters (Fred, Wilma), objects (blue hat, couch) and background (setting that resembles a living room); (b) \textbf{Layout Feasibility} - characters and objects must be placed at plausible locations and scales (Fred, Wilma and the couch should be placed on the ground plane, the hat must lie on top of Fred's head); (c) \textbf{Appearance Fidelity} - entity appearance, which may be affected by identity, pose, action, attributes and layout, should respect the scene description; (d) \textbf{Interaction Consistency} - appearance of characters and objects must be consistent with each other given the described, sometimes implicit, interaction (Fred and Wilma should face each other as do people when they talk to each other); (f) \textbf{Language Understanding} - the system must be able to understand and translate a natural language description into a plausible visual instantiation.

Currently, the dominant approaches to conditional generation of visual data from text rely on directly learning distributions in a high dimensional pixel space. While these approaches have shown impressive results for aligned images of objects (faces, birds, flowers, etc.), they are often inadequate for addressing the above challenges due to the combinatorial explosion of the image space arising from multiple characters and objects with significant appearance variations arranged in a large number of possible layouts. This is especially true when the only source of supervision is text-image pairs representing a sparse sample of the image space without rich semantic grounding of text elements in the image.

%{There has been a surge of interest within the computer vision community towards the generative modelling of visual data. Early approaches focused on unconditional image generation [refs], where as recent works have started exploring generative models conditioned on simple textual inputs describing objects and their appearances [refs]. While these approaches have shown good results for aligned images of objects (faces, birds, flowers, etc.), they are often inadequate at generating complex scenes, due to the combinatorial explosion of the image space arising from multiple characters and objects with significant appearance variations arranged in a large number of possible layouts.}

We introduce \taskfull\ (\task), the task of generating complex videos from rich natural language descriptions. \task\ models are trained using a densely annotated video dataset consisting of scene descriptions and bounding boxes for the mentioned characters and objects. During inference, the models must generate videos for novel descriptions (unseen in the training dataset). To quantitatively measure progress in \task\, we propose two sets of metrics. The first measures the \emph{semantic fidelity} of the generated video to the desired description using entity noun, adjective, and verb recalls. The second measures \emph{semantic consistency} capturing the consistency of the appearances, poses and layouts of entities with regards to other entities in the video as well as to the background.

We propose the \modelfull\ (\model) that explicitly models the spatio-temporal layout of characters and objects in the scene jointly with entity appearances. Unlike pixel generation approaches, our appearance model is based on text to entity segment retrieval from a video database. Spatio-temporal segments are extracted from the retrieved videos and fused together to generate the final video. The layout composition and entity retrieval work in a sequential manner which is determined by the language input. Factorization of our model into composition and retrieval stages alleviates the need to directly model pixel spaces, results in an architecture that more easily exploits location and appearance contextual cues (important for interaction consistency), and renders a more interpretable output.

Towards the goal of \task, we introduce \dataset, a densely annotated dataset based on The Flintstones animated series, consisting of over 25000 videos, each 75 frames long. \dataset\ has several advantages over using a random sample of videos that are available online. Firstly, in a closed world setting such as a television series, the most frequent characters are present in a wide variety of settings, which serves as a more manageable learning problem than a sparse set obtained in an open world setting. Secondly, the flat textures in animations are easier to model than real world videos. Thirdly, in comparison to other animated series, we found The Flintstones to have a good balance between having fairly complex interactions between characters and objects and yet not having overly complicated scenes with too much clutter. For these reasons, we believe that the \dataset\ dataset is semantically rich, preserves all the challenges of text to scene generation and is a good stepping stone towards real videos. \dataset\ consists of an $80$-$10$-$10$ train-val-test split. The train and val sets are used for learning and model selection respectively. Test captions serve as novel descriptions to generate videos at test time.

% This paragraph is IMPORTANT. We still need to copy paste sentences from here
%Motivated by recent advances in vision-language research, we also present a retrieval and composition approach to VSSG. Our complete system consists of a layout prediction model, a text to entity-video retrieval model, and a text to background-video retrieval model which are all trained in the learning phase. In the generation phase, entities are added to a retrieved background one by one in the order of appearance in the text description. At each iteration, the layout model predicts a location for an entity conditioned on the visual appearances and locations of previous entities. Given the predicted location and the video constructed so far, the current entity is retrieved from the database using text to video retrieval and added to the partially constructed video. This sequential approach is an approximation to joint location prediction and joint retrieval of all entities mentioned in the text. 

% ------ This paragraph has some good points ------
%{Maybe talk about this in the layout prediction and retrieval model section. Joint modelling of locations and appearance of all entities in a description presents fundamentally unique challenges for spatial and appearance knowledge representation beyond existing language-guided localization and image-retrieval tasks. \textit{First}, predicting plausible locations and scales for objects not yet in an image requires a significant amount of spatial knowledge about people and objects, in contrast to text based object localization which relies heavily on appearance cues. This includes knowledge like -- a hat usually goes on top of a person's head, a couch goes under the person sitting on it, a person being talked to faces the person speaking instead of facing away, tables have short and wide bounding boxes while standing people have tall and thin ones etc. \textit{Second}, retrieving an entity described in the text from a database of images for scene generation is also more complex than caption based image retrieval. Not only does the retrieved entity need to match the semantics of the description but it also needs to respect the implicit relational constraints or context imposed by the appearance and locations of other entities. For examples, for the description \emph{Fred is talking to Wilma}, it is not sufficient to retrieve \emph{a Wilma}, but one who is also facing in the right direction, i.e. towards \emph{Fred}.}

\ani{Now, talk about the results we obtain, and the ability of the model to generate videos for novel captions, as well as generalizing to a new dataset. Our results show that this architecture more easily exploits location and appearance contextual cues and outputs videos that have consistent layouts and appearances of characters and objects in accordance with the desired description.}

In summary, our contributions include: (a) The task of \taskfull, with a focus on the semantic fidelity to the description and consistent composition of the scene, with evaluation protocols to measure progress on both (b) A sequential inference approach and training procedure that jointly models the layout and appearances of entities in the scene described by a caption (c) The introduction of auxiliary classification losses based on the prediction of nouns, verbs and adjectives observed in the generated video, to supplement the more popular triplet loss (d) An explicit layout prediction model capable of learning and applying spatial world knowledge for creating feasible entity layouts (e) The \dataset\ dataset to study and make progress on the \task\ task.

%{This sequential approach is an approximation to jointly retrieving videos for all entities ($E_1,\cdots,E_n$) mentioned in the text $T$ that maximize a scoring function defined as $S(E_1,\cdots,E_n|T) \coloneqq S_1(E_1|T)\cdot S_2(E_2|E_1,T)\cdots S(E_n|E_1,\cdots,E_{n-1},T)$ by greedily maximizing the factors one at a time. Here a factor $S(E_i|E_1,\cdots,E_{i-1},T)$ measure the semantic and structural fitness or consistency of $E_i$ given the previous entity videos and the text.}
%{and composition approach to the task that allows us to sidestep the problem of learning distributions in high dimensional pixel space and focus on the semantic and structural consistency of the generated scene. While sharing some of the challenges of some existing vision-language localization and retrieval tasks, VSSG introduces some fundamentally unique challenges in spatial and appearance knowledge representation. \textbf{First}, consider predicting the location of an entity mentioned in the description in a partially constructed scene. Unlike existing language guided localization tasks which essentially boil down to predicting an object appearance template from text and pattern matching against the input image, predicting location for an object not yet in the image relies heavily on prior knowledge about locations and shapes of different entities and their spatial relations. This includes knowledge like -- a hat usually goes on top of a person's head, a couch goes under the person sitting on it, a person being talked to goes in front of the person speaking instead of behind him, tables have short and wide bounding boxes while standing people have tall and thin ones etc. \textbf{Second}, retrieving an entity described in the text from a database of images for scene generation is also more complex than caption-image retrieval. Not only does the retrieved entity need to match the semantics of the description but it also needs to respect the implicit relational constraints or context imposed by appearance and locations of other entities. For examples, for the description \emph{Fred is talking to Wilma}, it is not sufficient to retrieve \emph{a Wilma}, but one who is also facing in the right direction, i.e. towards \emph{Fred}.}


%\begin{enumerate}
%    \item (Need to concretize this idea) From a research perspective, this is also challenging. Where does one acquire the necessary knowledge ? How does one define good metrics ? How does one acquire and use a large dataset for this purpose ?
%    \item We propose the task of VSSG, the task of generating rich and complex video scenes from natural language descriptions. Knowledge acquisition is done using a densely annotated training dataset. Generation has access to database of videos without any text annotations, allowing retrieval methods to .... + Dataset overview
%    \item We propose the following metrics ...
%    \item Model overview
%    \item Results. Ablation. Generalization.
%    \item Why is this task more complex / better than other tasks ?
%\end{enumerate}

==> sections/introduction_bkp.tex <==
\section{Introduction}
Consider the scene description: \emph{Fred is talking to Wilma in the living room. Wilma is sitting on the couch}. Picturing the scene in our mind requires the knowledge of plausible locations, appearances, actions, and interactions of characters and objects being described. It also demands the ability to understand and translate the natural language description into a plausible visual instantiation. In this work, our goal is to build a model that replicates this ability to acquire visually grounded semantic and spatial knowledge and then apply it while generating plausible videos for novel text descriptions.

The vision community has shown tremendous interest in modelling the conditional distribution of images or videos given a text description in a \textit{high dimensional pixel space}. This approach has led to impressive performance on centered and aligned images of objects belonging to a few classes (birds, flowers, faces etc.) with limited spatial and appearance variations. However, this approach is inadequate for handling complex scenes due to the combinatorial explosion of the image space arising from multiple characters and objects with significant appearance variations arranged in a large number of possible layouts.

We propose the task of Visual Semantic Scene Generation (VSSG) where the focus is on generating complex video scenes from text. The task setup consists of two stages. First, during the \textit{learning} phase, a model acquires visually grounded semantic world knowledge from paired and richly annotated video-caption training data. Then during the \textit{generation} phase the model must use the learned knowledge to create a video for a novel caption by using a database of videos \textit{without} any text annotations. 

To study the task and measure progress, we introduce a dataset based on The Flintstones Animated series. The dataset consists of over 25000 videos, each 3 sec. or 75 frames long, annotated with character-centric captions. We use an $80$-$10$-$10$ train-val-test split. The train and val sets are used for learning and model selection respectively during the learning phase. Test captions serve as novel descriptions to generate videos for during the generation phase with test set videos acting as the unannotated visual database. The text annotations for test set videos are used for automated semantic evaluation in addition to human evaluations that measure semantic fidelity to the description and visual quality.  

Motivated by recent advances in vision-language research, we also present a retrieval and composition approach to VSSG. Our complete system consists of a layout prediction model, a text to entity-video retrieval model, and a text to background-video retrieval model which are all trained in the learning phase. In the generation phase, entities are added to a retrieved background one by one in the order of appearance in the text description. At each iteration, the layout model predicts a location for an entity conditioned on the visual appearances and locations of previous entities. Given the predicted location and the video constructed so far, the current entity is retrieved from the database using text to video retrieval and added to the partially constructed video. This sequential approach is an approximation to joint location prediction and joint retrieval of all entities mentioned in the text. 

Joint modelling of locations and appearance of all entities in a description for VSSG presents fundamentally unique challenges for spatial and appearance knowledge representation not found in existing language-guided localization and image-retrieval tasks. \textit{First}, predicting a plausible location and scale for an object not yet in an image relies a lot more on prior spatial knowledge than text based object localization in an image which relies heavily on appearance cues. This includes knowledge like -- a hat usually goes on top of a person's head, a couch goes under the person sitting on it, a person being talked to goes in front of the person speaking instead of behind him, tables have short and wide bounding boxes while standing people have tall and thin ones etc. \textit{Second}, retrieving an entity described in the text from a database of images for scene generation is also more complex than caption-image retrieval. Not only does the retrieved entity need to match the semantics of the description but it also needs to respect the implicit relational constraints or context imposed by appearance and locations of other entities. For examples, for the description \emph{Fred is talking to Wilma}, it is not sufficient to retrieve \emph{a Wilma}, but one who is also facing in the right direction, i.e. towards \emph{Fred}.

%{This sequential approach is an approximation to jointly retrieving videos for all entities ($E_1,\cdots,E_n$) mentioned in the text $T$ that maximize a scoring function defined as $S(E_1,\cdots,E_n|T) \coloneqq S_1(E_1|T)\cdot S_2(E_2|E_1,T)\cdots S(E_n|E_1,\cdots,E_{n-1},T)$ by greedily maximizing the factors one at a time. Here a factor $S(E_i|E_1,\cdots,E_{i-1},T)$ measure the semantic and structural fitness or consistency of $E_i$ given the previous entity videos and the text.}
%{and composition approach to the task that allows us to sidestep the problem of learning distributions in high dimensional pixel space and focus on the semantic and structural consistency of the generated scene. While sharing some of the challenges of some existing vision-language localization and retrieval tasks, VSSG introduces some fundamentally unique challenges in spatial and appearance knowledge representation. \textbf{First}, consider predicting the location of an entity mentioned in the description in a partially constructed scene. Unlike existing language guided localization tasks which essentially boil down to predicting an object appearance template from text and pattern matching against the input image, predicting location for an object not yet in the image relies heavily on prior knowledge about locations and shapes of different entities and their spatial relations. This includes knowledge like -- a hat usually goes on top of a person's head, a couch goes under the person sitting on it, a person being talked to goes in front of the person speaking instead of behind him, tables have short and wide bounding boxes while standing people have tall and thin ones etc. \textbf{Second}, retrieving an entity described in the text from a database of images for scene generation is also more complex than caption-image retrieval. Not only does the retrieved entity need to match the semantics of the description but it also needs to respect the implicit relational constraints or context imposed by appearance and locations of other entities. For examples, for the description \emph{Fred is talking to Wilma}, it is not sufficient to retrieve \emph{a Wilma}, but one who is also facing in the right direction, i.e. towards \emph{Fred}.}

\hline

\begin{enumerate}
    \item There has been a surge of interest in generative modelling of visual data. While early approaches focused on unconditional image generation, recent works have started exploring generative models conditioned on simple text descriptions such as .... 
    \item Consider a rich scene description ..... (Maybe add a slightly more complex example).
    \item Generating a video given this description poses several challenges:\\
    1. Plausible locations (give examples)\\
    2. Appearances\\
    3. Actions\\
    4. Interactions\\
    5. Parsing natural language\\
    \item (Need to concretize this idea) From a research perspective, this is also challenging. Where does one acquire the necessary knowledge ? How does one define good metrics ? How does one acquire and use a large dataset for this purpose ?
    \item We propose the task of VSSG, the task of generating rich and complex video scenes from natural language descriptions. Knowledge acquisition is done using a densely annotated training dataset. Generation has access to database of videos without any text annotations, allowing retrieval methods to .... + Dataset overview
    \item We propose the following metrics ...
    \item Model overview
    \item Why is this task more complex / better than other tasks ?
\end{enumerate}


==> sections/layout_predictor.tex <==
\section{Layout predictor}
\input{figures/layout_predictor.tex}
The layout predictor models $P(l_i|V_{i-1},T,e_i;\theta_{loc},\theta_{scale})$, the conditional distribution of position of $i^{th}$ entity given the text, entity noun position in tokenized text, and the partial video with previous entities. Let $C_i$ denote the conditioning information, $(V_{i-1},T,e_i)$. We factorize the distribution as follows
\begin{equation}
P(l_i|C_i;\theta_{loc},\theta_{scale}) = \prod_{f=1}^{F} P_{loc}^f(x_{if},y_{if}|C_i;\theta_{loc}^f)\cdot P_{scale}^f(w_{if},h_{if}|x_{if},y_{if},C_i;\theta_{scale}^f)
\end{equation}
where $\theta_{loc}=\{\theta_{loc}^f\}_{f=1}^{F}$ and $\theta_{scale}=\{\theta_{scale}^f\}_{f=1}^{F}$ are learnable parameters. 

$P_{loc}^f$ is modelled using a network that takes $C_i$ as input and produces a distribution over all pixel locations for $f^{th}$ image frame. We represent $P_{scale}^f$ using a Gaussian distribution whose mean and covariance are predicted using a network given 
$(x_i,y_i,C_i)$. Hence,
\begin{multline}
P_{scale}^f(w_{if},h_{if}|x_{if},y_{if},C_i;\theta_{scale}^f) = \\ \mathcal{N}(w_{if},h_{if}|\mu(x_{if},y_{if},C_i;\theta_{scale}^f),\Sigma(x_{if},y_{if},C_i;\theta_{scale}^f))
\end{multline}
where $\mu^f(\cdot) \in \mathbb{R}^2$ and $\Sigma^f(\cdot) \in \mathbb{R}^{2\times 2}$. Network parameters $\theta_{loc}$ and $\theta_{scale}$ are learned from ground truth position annotations by maximum likelihood estimation by minimizing the following loss
\begin{multline}\label{eq:mle_loss}
\sum_{m=1}^{M}\sum_{i=1}^{n^{[m]}}\sum_{f=1}^{F}\left[-\log(P_{loc}^f(x_{if}^{[m]},y_{if}^{[m]}|C_i^{[m]};\theta_{loc}^f)) \; + \right. \\
\left. 0.5 \cdot (z_{if}^{[m]}-\mu(x_{if}^{[m]},y_{if}^{[m]},C_i^{[m]};\theta_{scale}^f))^T\Sigma^{-1}(z_{if}^{[m]}-\mu(x_{if}^{[m]},y_{if}^{[m]},C_i^{[m]};\theta_{scale}^f)) \; + \right. \\
\left. \log(2\pi) + 0.5 \cdot  \log(\det(\Sigma(x_{if},y_{if},C_i;\theta_{scale}^f))) 
\right]
\end{multline}
where $z_{if}=[w_{if};h_{if}]$. For simplicity, we manually set and freeze $\Sigma$ to a diagonal covariance matrix in all our experiments. 

\subsection{Layout Predictor Network Architecture} 

\subsubsection{Feature Computation Backbone.} Both $P_{loc}^f$ and $\mu^f$ have an identical feature computation backbone comprising of a CNN and a bidirectional LSTM. The CNN encodes $V_{i-1}$ (8 sub-sampled frames concatenated along the channel dimension) as a set of convolutional feature maps which capture appearance and positions of previous entities in the scene. The LSTM is used to encode the entity $E_i$ for which the prediction is to be made along with semantic context available in the caption. The caption is fed into the LSTM and the hidden output at $e_i^{th}$ word position is extracted as the entity text encoding. The text encoding is replicated spatially and concatenated with convolutional features and 2-D grid coordinates to create a representation for each location in the convolutional feature grid that is aware of visual, spatial, temporal, and semantic context.

\subsubsection{Location Predictor.} In $P_{loc}^f$, an MLP produces a score for each location. The score feature map is bilinearly upsampled to the size of input video frames. Then, a softmax layer over all pixels produces $P_{loc}^f(x,y|C;\theta_{loc}^f)$ for every pixel location $(x,y)$ in the $f^{th}$ video frame.

\subsubsection{Scale Predictor.} In $\mu^f$, the features computed by the backbone at a particular $(x,y)$ location are selected and fed into the scale MLP that produces $\mu^f(x,y,C_i;\theta_{scale}^f)$.

\subsubsection{Feature sharing and multitask training.} While it is possible to train a separate network for each $\{P_{loc}^f,\mu^f\}_{f=1}^F$, we present a pragmatic way of sharing features and computation for different frames and also between the location and scale networks. 

To share features and computation across frames, the location network produces $F$ probability maps in a single forward pass. This is equivalent to sharing all layers across all $P_{loc}^f$ nets except for the last layer of the MLP that produces location scores. Similarly, all $\mu^f$ nets are combined into a single network that produces $F$ $(\mu_w,\mu_h)$ pairs. We refer to the combined networks by $P_{loc}$ and $\mu$.

In addition, we also share features across location and scale networks. First, we share the feature computation backbone, the output from which is then passed into location and scale specific layers. Second, we use a soft-attention mechanism to select likely positions for feeding into the scale layers. We combine the $F$ spatial maps into a single attention map through max pooling. This attention map is used to perform weighted average pooling on backbone features which are then fed into the scale MLP. Note that this is a differentiable greedy approximation to find the most likely location (by taking argmax of spatial probability maps) and scale (using output of $\mu$ directly) in a single forward pass. To keep training consistent with inference, we use the soft-attention mechanism instead of feeding ground-truth locations into $\mu$. The parameters are learned by minimizing equation~\eqref{eq:mle_loss} through mini-batch gradient descent using the Adam optimizer.

==> sections/task_overview.tex <==
\section{Visual Semantic Scene Generation}
The task of VSSG consists of two phases - (i) learning visually grounded semantic knowledge about the world from paired and richly annotated video-caption training data, and (ii) generating videos for novel captions given a database of videos without any text annotations. 

\subsubsection{Learning Phase.} Generating a plausible visual instantiation of a scene described in natural language not only requires an understanding of how visual representation of a scene translates into a text description and vice versa, but it also requires a great deal of spatial and visual knowledge about the world. \emph{Spatial knowledge} comprises of knowledge of feasible locations and scales of an entity in the described scene. \emph{Visual knowledge} consists of appearance of entities affected by actions and attributes. The learning phase deals with acquiring this knowledge from training data consisting of videos annotated with text descriptions and bounding box trajectories of each noun chunk in the description. 

\subsubsection{Generation Phase.} This phase aims to apply the learned knowledge for creating a video from a novel text description with the help of database of unannotated videos. Restricting the generation phase to unannotated videos has two advantages. First, it allows testing of the generalization ability of the learned visual knowledge. Second, it is a more practical and scalable paradigm which avoids expensive and time consuming video text annotations.

==> tables/stage2_feature_ablation_gt.tex <==
\setlength{\tabcolsep}{4pt}
\begin{table}
\begin{center}
\caption{\textbf{Entity retriever feature ablation with GT previous entities.} Extent to which the entity retriever uses text, image, and coordinate features when using \textbf{ground truth} previous entity positions and appearances shown using leave-one-out ablation}
\label{table:stage2_feature_ablation_gt}
\begin{tabular}{ccccccccc}
\hline\noalign{\smallskip}
& & & \multicolumn{3}{c}{\textbf{Recall@}1}   & \multicolumn{3}{c}{\textbf{Recall@10}}              \\ \cmidrule{4-9}
\textbf{Text}   &   \textbf{Image}  &   \textbf{Coord.} & \textbf{Noun}  & \textbf{Adj.}   & \textbf{Verb}      & \textbf{Noun}  & \textbf{Adj.}   & \textbf{Verb}  \\
\noalign{\smallskip}
\hline
  & \checkmark & \checkmark & 62.23 & 54.18 & 47.50  & 92.38 & 88.21 & 92.13       \\
\checkmark &   & \checkmark     & 54.32 & 14.83 & 10.37 & 74.88 & 56.84 & 47.05 \\
\checkmark & \checkmark &       & 76.16 & 52.47 & 51.51 & 94.20  & 88.97 & 92.22 \\ \hline
\checkmark & \checkmark & \checkmark     & 76.88 & 55.51 & 52.58 & 94.74 & 92.01 & 93.52 \\
\end{tabular}
\end{center}
\end{table}
\setlength{\tabcolsep}{1.4pt}






==> tables/stage2_feature_ablation_q_test_db_test.tex <==
\setlength{\tabcolsep}{4pt}
\begin{table}
\begin{center}
\caption{\textbf{Entity retriever feature ablation.} Extent to which the entity retriever uses text, image, and coordinate features shown using leave-one-out ablation. When using GT previous entities, all features are used by the model. When using predicted previous entities, dropping image features leads to performance improvement. We believe, since the model has been trained with ground truth entity appearances only, the learned query embedding model is not robust to errors in retrieval of previous entities.}
\label{table:stage2_feature_ablation_gt}
\begin{subtable}{1\textwidth}
\centering
\caption{(a) With \textbf{ground truth} positions and appearances of previous entities}
\begin{tabular}{ccccccccc}
\hline\noalign{\smallskip}
& & & \multicolumn{3}{c}{\textbf{Recall@}1}   & \multicolumn{3}{c}{\textbf{Recall@10}}              \\ \cmidrule{4-9}
\textbf{Text}   &   \textbf{Image}  &   \textbf{Coord.} & \textbf{Noun}  & \textbf{Adj.}   & \textbf{Verb}      & \textbf{Noun}  & \textbf{Adj.}   & \textbf{Verb}  \\
\noalign{\smallskip}
\hline
  & \checkmark & \checkmark & 62.23 & 54.18 & 47.50  & 92.38 & 88.21 & 92.13       \\
\checkmark &   & \checkmark     & 54.32 & 14.83 & 10.37 & 74.88 & 56.84 & 47.05 \\
\checkmark & \checkmark &       & 76.16 & 52.47 & 51.51 & 94.20  & 88.97 & 92.22 \\ \hline
\checkmark & \checkmark & \checkmark     & 76.88 & 55.51 & 52.58 & 94.74 & 92.01 & 93.52 \\
\end{tabular}
\end{subtable}

\begin{subtable}{1\textwidth}
\centering
\caption{(b) With \textbf{predicted} positions and appearances of previous entities}
\begin{tabular}{ccccccccc}
\hline\noalign{\smallskip}
& & & \multicolumn{3}{c}{\textbf{Recall@}1}   & \multicolumn{3}{c}{\textbf{Recall@10}}              \\ \cmidrule{4-9}
\textbf{Text}   &   \textbf{Image}  &   \textbf{Coord.} & \textbf{Noun}  & \textbf{Adj.}   & \textbf{Verb}      & \textbf{Noun}  & \textbf{Adj.}   & \textbf{Verb}  \\
\noalign{\smallskip}
\hline
  & \checkmark & \checkmark & 26.41 & 4.37  & 9.03  & 55.67 & 19.39 & 37.6      \\
\checkmark &   & \checkmark     & 54.32 & 14.83 & 10.37 & 74.88 & 56.84 & 47.05 \\
\checkmark & \checkmark &       & 51.69 & 9.88  & 8.54  & 67.71 & 37.45 & 41.13 \\ \hline
\checkmark & \checkmark & \checkmark     & 52.72 & 12.17 & 8.64  & 68.61 & 37.83 & 41.38 \\
\end{tabular}
\end{subtable}
\end{center}
\end{table}
\setlength{\tabcolsep}{1.4pt}

==> tables/stage2_feature_ablation_q_test_db_train.tex <==
\setlength{\tabcolsep}{4pt}
\begin{table}
\begin{center}
\caption{\textbf{Entity retriever feature ablation.} Extent to which the entity retriever uses text, image, and coordinate features shown using leave-one-out ablation. When using GT previous entities, all features are used by the model. When using predicted previous entities, dropping image features leads to performance improvement. We believe, since the model has been trained with ground truth entity appearances only, the learned query embedding model is not robust to errors in retrieval of previous entities.}
\label{table:stage2_feature_ablation_gt}
\begin{subtable}{1\textwidth}
\centering
\caption{(a) With \textbf{ground truth} positions and appearances of previous entities}
\begin{tabular}{ccccccccc}
\hline\noalign{\smallskip}
& & & \multicolumn{3}{c}{\textbf{Recall@}1}   & \multicolumn{3}{c}{\textbf{Recall@10}}              \\ \cmidrule{4-9}
\textbf{Text}   &   \textbf{Image}  &   \textbf{Coord.} & \textbf{Noun}  & \textbf{Adj.}   & \textbf{Verb}      & \textbf{Noun}  & \textbf{Adj.}   & \textbf{Verb}  \\
\noalign{\smallskip}
\hline
         & \checkmark & \checkmark & 27.44 & 8.17  & 7.54  & 58.11 & 26.24 & 36.04 \\
\checkmark &          & \checkmark & 60.54 & 9.5   & 11.2  & 77.71 & 39.92 & 43.58 \\
\checkmark & \checkmark &           & 56.11 & 12.93 & 10.64 & 72.61 & 43.16 & 41.21 \\ \hline
\checkmark & \checkmark & \checkmark & 59.68 & 17.68 & 13.71 & 75.19 & 51.52 & 45.17 \\ \hline
\end{tabular}
\end{subtable}

\begin{subtable}{1\textwidth}
\centering
\caption{(b) With \textbf{predicted} positions and appearances of previous entities}
\begin{tabular}{ccccccccc}
\hline\noalign{\smallskip}
& & & \multicolumn{3}{c}{\textbf{Recall@}1}   & \multicolumn{3}{c}{\textbf{Recall@10}}              \\ \cmidrule{4-9}
\textbf{Text}   &   \textbf{Image}  &   \textbf{Coord.} & \textbf{Noun}  & \textbf{Adj.}   & \textbf{Verb}      & \textbf{Noun}  & \textbf{Adj.}   & \textbf{Verb}  \\
\noalign{\smallskip}
\hline
          & \checkmark & \checkmark & 24.88 & 3.04  & 9.48  & 55.22 & 19.39 & 37.18 \\
\checkmark &           & \checkmark & 60.54 & 9.5   & 11.2  & 77.71 & 39.92 & 43.58 \\
\checkmark & \checkmark &           & 56.14 & 8.56  & 11.34 & 73.03 & 39.35 & 41.48 \\ \hline
\checkmark & \checkmark & \checkmark & 61.19 & 12.36 & 14.77 & 75.98 & 47.72 & 46.86\\ \hline
\end{tabular}
\end{subtable}
\end{center}
\end{table}
\setlength{\tabcolsep}{1.4pt}
